SwiftCache: Model-Based Learning for Dynamic Content Caching in CDNs

We introduce SwiftCache, a "fresh" learning-based caching framework designed for content distribution networks (CDNs) featuring distributed front-end local caches and a dynamic back-end database. Users prefer the most recent version of the dynamically updated content, while the local caches lack knowledge of item popularity and refresh rates. We first explore scenarios with requests arriving at a local cache following a Poisson process, whereby we prove that the optimal policy features a threshold-based structure with updates occurring solely at request arrivals. Leveraging these findings, SwiftCache is proposed as a model-based learning framework for dynamic content caching. The simulation demonstrates near-optimal cost for Poisson process arrivals and strong performance with limited cache sizes. For more general environments, we present a model-free Reinforcement Learning (RL) based caching policy without prior statistical assumptions. The model-based policy performs well compared to the model-free policy when the variance of interarrival times remains moderate. However, as the variance increases, RL slightly outperforms model-based learning at the cost of longer training times, and higher computational resource consumption. Model-based learning's adaptability to environmental changes without retraining positions it as a practical choice for dynamic network environments. Distributed edge caches can utilize this approach in a decentralized manner to effectively meet the evolving behaviors of users.

==> to_be_deleted.tex <==

\title{Learning-Based Fresh Caching for CDNs: Efficiency and  Adaptability} 



\begin{abstract}
We consider a "fresh" learning-based caching framework for content distribution networks (CDNs) with distributed front-end local caches and a dynamic back-end database. The users prefer the most recent version of the dynamically updated content, while the local caches lack knowledge of item popularity and refresh rates. We first explore scenarios with requests arriving at a local cache following a Poisson process, whereby we prove that the optimal policy features a threshold-based structure. Based on this foundation, we propose a model-based learning algorithm for caching dynamic content. The simulation demonstrates near-optimal cost for Poisson process arrivals and strong performance with limited cache sizes. For more general environments, we present a model-free Reinforcement Learning (RL) based caching policy without prior statistical assumptions. The model-based policy performs well compared to the model-free policy when the variance of interarrival times remains moderate. However, as the variance increases, RL slightly outperforms model-based learning at the cost of longer training times, and higher computational resource consumption. Model-based learning's quick adaptability to environmental changes and its fast convergence rate, makes it a desirable approach for dynamic network environments. This framework offers efficient fresh caching solutions for content distribution networks.
\end{abstract}




\section{Introduction}
Content distribution networks (CDNs) are crucial for efficiently delivering content to users while improving overall performance and reducing network congestion \cite{vakali2003content, llorca2013dynamic, buyya2008content, bartolini2003optimal}. In the era of 5G networks, caching at the wireless edge is employed to accelerate content downloads and enhance wireless network performance \cite{liu2016caching, yao2019mobile, paschos2018role, zhang2018cooperative}.

However, the emergence of new services like video on demand, augmented reality, social networking, and online gaming, which produce constantly changing data, has rendered traditional caching methods less efficient. The importance of content freshness has grown significantly due to the rapid increase in mobile devices and real-time applications like video on demand and live broadcast \cite{zhang2019price}. Simply serving content to users is no longer sufficient, as users prefer the latest data versions, valuing fresh content the most \cite{shapiro1998information}. Directly delivering the freshest content from the back-end database to users can congest the network and degrade the quality of experience (QoE). These challenges are amplified with the growth of cellular traffic in the network. Consequently, there is a pressing need to develop new caching strategies that consider content refresh characteristics and aging costs to ensure efficient dynamic content distribution.


The dynamic nature of content in CDNs necessitates the implementation of effective caching strategies to maintain the freshness of cached content \cite{zhang2018towards, yan2021learning}. This is crucial to enable users to access the most up-to-date information, especially in rapidly evolving environments where content popularity, demand intensity, and refresh rates are constantly fluctuating \cite{li2016popularity, kam2017information}. 


Numerous works study the dynamic content delivery in caching systems such as \cite{najm2016age, candan2001enabling, shi2002workload, li2003freshness, wu2019dynamic, kam2017information, xu2020proactive, gao2020design, abolhassani2020achieving, mehrizi2019popularity, kumar2020optimized, zhong2018two, zhang2020reinforcement, masood2020learning, azimi2018online, zhang2019learning, abad2019dynamic} and effective strategies have been proposed. Existing works have studied metrics like "age of synchronization" (AoS) and "age of information" (AoI) for measuring cached content freshness \cite{zhong2018two, kam2017information}. However, real-world scenarios may require a different metric, "Age-of-Version" (AoV), which considers the version difference between database and cache \cite{abolhassani2021fresh, abolhassani2023optimal, abolhassani2022fresh}. 


Despite the traditional caching paradigms, for content with varying generation dynamics, it is essential to regularly update the cached content \cite{amadeo2020caching, bastopcu2020maximizing}.  This is necessary to avoid the cache becoming outdated due to old content. The widespread deployment of edge caches across the network makes it impractical for the back-end database to manage and track all these caches, along with their content and ages. Thus, each individual edge cache takes on the responsibility of ensuring its cached content remains up-to-date and fresh. Edge caches must also consider the cost incurred by excessive cache updates to find a balance between content freshness and fetching costs. However, a significant challenge arises as these edge caches often lack access to network parameters in their deployment environment, such as item popularity profiles, refresh rates, and demand intensity. Thus, they need to learn these system parameters and develop strategies to manage cache updates effectively while keeping costs low. To achieve this, edge caches need to observe the environment and devise optimal policies for cache updates at any given moment.

Machine Learning techniques have been widely utilized in network environments to achieve optimal caching performance \cite{sethumurugan2021designing, chang2018learn, shuja2021applying}. Notably, Reinforcement Learning (RL) proves to be a viable option for edge caches, allowing them to learn user behavior through observing and interacting with them \cite{shuja2021applying, zhu2018deep, jiang2019multi}. The rate at which users generate requests can significantly impact the time required for the RL policy to gather sufficient data and accurately learn the environment. Additionally, when the environment undergoes changes, such as shifts in popularity or refresh rates, retraining becomes necessary as the older policy may no longer be suitable for the new environment. This can demand substantial computational resources at the edge caches which may exceed their available capacity. These challenges highlight the need for adaptable and efficient learning algorithms that can quickly adjust to changing conditions and ensure optimal caching performance in dynamic network environments.





In this study, we address the challenging problem of caching dynamic content in the most general setting, where local caches lack knowledge of item popularity, demand intensity, and refresh rates. To overcome these limitations and devise a more adaptable caching framework, we propose a "fresh" learning-based approach. We begin by investigating the scenario where requests arrive at local caches following a Poisson process, and demonstrate that under certain conditions, the optimal policy takes on a threshold-based structure. Leveraging insights gained from this optimal policy, we introduce a model-based learning algorithm that efficiently manages limited cache capacity and eliminates the need for resource-intensive training. Moving beyond the constraints of the Poisson process, we further explore Reinforcement Learning (RL) as a viable caching policy for more general environments. While the RL approach offers adaptability to diverse environments, it requires longer training times and higher computational resource consumption compared to model-based learning.

To assess the performance of our proposed framework, we conduct extensive simulations and evaluate its cost-effectiveness compared to the optimal caching policy. Our results demonstrate that model-based learning emerges as a solid caching framework, achieving near-optimal cost and exhibiting resilience to environmental changes without the need for extensive computational resources. 

The rest of the paper is organized as follows. In Section~\ref{sec:Sys_Model}, we present a practical caching model for efficient dynamic content delivery with minimized long-term average costs. Section~\ref{sec: optimal-policy} identifies optimal caching policies in Poisson Process-based scenarios, revealing threshold-based structures. Building on these insights, Section~\ref{sec:model-based} introduces a model-based learning algorithm achieving near-optimal cost without knowledge of item popularity and refresh rates. In Section~\ref{sec:Model_free}, we propose a model-free reinforcement learning and compare it to our proposed algorithm highlighting their respective strengths and trade-offs. And finally we conclude the paper in Section~ \ref{sec:conclusion}.


\section{System Model}
The hierarchical caching system depicted in Fig.~\ref{fig:system,model} is designed to serve a user population with dynamic content. Requests arrive at the local cache with an intensity represented by the rate parameter $\beta\geq0$. The size of data items is denoted as $(b_n)_{n=1}^N$, and the popularity profile is characterized by $\mathbf{p}=(p_n)_{n=1}^N$. Updates for each data item occur at an average rate of $\lambda_n\geq 0$ updates per second, represented by the vector $\boldsymbol{\lambda}=(\lambda_n)_{n=1}^N$. Notably, the local cache which has a limited cash capacity, lacks knowledge of the popularity profile $\mathbf{p}$ and refresh rate $\boldsymbol{\lambda}$.


\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{System_Model.pdf}
\caption{Setting of \textit{Fresh Caching for Dynamic Content}}
\label{fig:system,model}
\end{figure}

\noindent\textbf{Age Dynamics: }To quantify freshness, we use the \emph{Age-of-Version} $\Delta_n(t)$, representing the number of updates since the item was last cached \cite{abolhassani2021fresh}.\\
\textbf{Fetching and Aging Costs: }Operational costs include fetching an item of size $b_n$ that incures cost $b_n \,c_f>0$. Performance costs account for serving an item with age $\Delta_n(t)$, incurring a freshness cost of $c_a \times \Delta_n(t)$.

\noindent \textbf{Problem Statement:} 
Our main goal is to develop efficient caching strategies that strike the right balance between the costs of frequently updating local content and providing aged content to users. Specifically, we seek a policy that minimizes the long-term average cost by making decisions on cache updates and request serving from the edge-cache. This objective can be formulated as follows:
\begin{equation}
\label{eq:costproblem}
\begin{split}
    &\min _{\boldsymbol{u}} \lim _{\mathrm{T} \rightarrow \infty} \frac{1}{T} \mathbb{E}_{s}^{u}\left[\int_{o}^{\mathrm{T}} \sum_{n=1}^N C_{n}^{\pi}\left(s_{n}(t),u_n(t)\right) dt\right]\\
    & s.t. \quad  u_n(t) \in \{0,1\}, \quad \forall n \in \cN , t\geq 0,
\end{split}
\end{equation}
where $u_n(t)\in \{0,1\}$ and $s_n(t)$ represent the action and state of the system at time $t$ for data item $n$, respectively. The cost of the system for data item $n$ at time $t$, given the state $s_n(t)$ and action $u_n(t)$ under a particular paradigm $\pi$, is denoted as $C_{n}^{\pi}\left(x_n(t),u_n(t)\right)$. The operator $\mathbb{E}_{s}^{u}$ captures the expected value over the system state $s$ for a given action $u$.
Our aim is to find the optimal policy $\boldsymbol{u}$ that minimizes this long-term average cost. 


To address the challenges of the general problem expressed in \ref{eq:costproblem}, we first focus on a specific scenario where the arrival requests follow a Poisson Process. In addition, we assume that the local cache possesses information about item popularity, refresh rates, and demand intensity. These assumptions enable us to analyze the optimal policy's structure, which will be discussed in the next section. 


\section{The Optimal Policy}
\label{sec: optimal-policy}

In this section, we focus on the previously introduced problem. Our goal is to analyze the structure of the optimal policy in a scenario where requests follow a Poisson process with a known rate $\beta$, and the local cache, constrained by limited storage capacity, is equipped with information about the popularity profile $\mathbf{p}$ and refresh rate $\boldsymbol{\lambda}$. Under these conditions, we present a clear characterization of the optimal policy in the following theorem.


\begin{theorem}
Consider a system comprising a dataset $\mathcal{N}$ of $N$ dynamic items, where each item has a corresponding size denoted as $(\boldsymbol{b})_{n=1}^N$. In this system, a local cache with a constraint on its average cache occupancy $\tilde{B}$ serves a group of users that generate demand according to a Poisson Process with a known rate $\beta$. The local cache possesses knowledge of the popularity profile $\mathbf{p}=(p_n)_{n=1}^N$ and refresh rates $\boldsymbol{\lambda}=(\lambda_n)_{n=1}^N$. Under these conditions, the optimal caching strategy is an eviction-based policy. Specifically, the local cache assigns a constant timer to each item upon its storage, and the item is evicted from the cache when the timer expires. The timers for each item are determined as follows:
As evident from Equation \ref{eq:solutiont}, the timers can be explicitly determined as a function of the system parameters, including the popularity, refresh rate, and size of the items. The parameter $\tilde{\alpha}$ is selected such that the constraint $\tilde{B}$ on the average cache occupancy is satisfied. The optimal value $\tilde{\alpha}^*$ exhibits an inverse relationship with $\tilde{B}$. As the cache capacity increases, $\tilde{\alpha}^*$ tends to approach zero. In the specific scenario of an unlimited cache capacity, this corresponds to setting $\tilde{\alpha}^* = 0$.

The following proposition provides a characterization of the optimal cost when the cache capacity is unlimited. We will utilize this cost as a benchmark for comparing the performance of our proposed algorithms. 

While Proposition \ref{prop:optimal_unlimited} provides the optimal cost under unlimited cache capacity, in real-world scenarios, cache occupancy is inherently limited due to dynamic content. Periodic updates are necessary to minimize freshness costs. The optimal policy's eviction-based structure achieves this by briefly retaining each item before eviction, resulting in a decrease in cache occupancy as content becomes more dynamic.
The insights from Theorem \ref{thm:optimalpolicy} rely on the assumption that the local cache has complete knowledge of demand intensity, popularity profile, and refresh rates. In practice, such comprehensive knowledge is often unavailable, and these parameters can change. In the next section, leveraging the insights from Theorem \ref{thm:optimalpolicy}, we propose a learning-based algorithm grounded in the eviction-based model. This algorithm eliminates the need for computationally demanding training procedures, saving computational resources. Additionally, its adaptability to dynamic system parameters ensures robustness in the face of changes, making it a practical and efficient solution.
\section{Model-Based Learning} 
In this section, we focus on crafting an efficient caching policy for dynamic content, where requests follow a Poisson process. Despite lacking information on popularity, refresh rates, and demand intensity, our goal is to design a policy that adapts to changing environmental conditions. Our proposed dynamic caching policy continuously learns and adjusts to evolving popularity and refresh rates, minimizing long-term average costs and achieving near-optimal performance in dynamic content caching.
Drawing insights from Theorem \ref{thm:optimalpolicy}, we introduce Algorithm 1, a model-based caching policy for dynamic content. Inspired by Theorem \ref{thm:optimalpolicy}, our proposed caching policy features an eviction-based structure, dynamically learning and adjusting timers to maintain average cache occupancy below a specified threshold while minimizing the average long-term costs.
The proposed algorithm employs three parameters—last request time of items ($\boldsymbol{\Bar{s}}$), last fetch time of items ($\boldsymbol{\Bar{t}}$), and the corresponding age of items during the last fetch ($\boldsymbol{\Delta}$)—to effectively manage the caching process. By monitoring and utilizing these parameters, the algorithm optimizes the caching strategy for efficient content delivery. To achieve this, the algorithm estimates refresh rates ($\hat{\boldsymbol{\lambda}}$) and interarrival times ($\boldsymbol{eit}$), utilizing them to calculate timers ($\boldsymbol{\tau}$) for each item. Specifically, the algorithm calculates the holding time $\tau_n$ for data item $n$ based on the estimated refresh rate $\hat{\lambda}_n$ and estimated interarrival times $eit_n$ as given by:
This calculation is rooted in the optimal policy provided in Theorem \ref{thm:optimalpolicy}. Additionally, the algorithm dynamically adjusts timer values to minimize costs while adhering to the cache occupancy constraint. This adaptive approach ensures an optimized caching strategy, even in the presence of fluctuations in popularity, refresh rates, and demand intensity. By actively adapting to these changes, the algorithm effectively handles the dynamic nature of the system, ensuring efficient and robust performance.
To assess our algorithm's performance against the benchmark cost outlined in Proposition \ref{prop:optimal_unlimited}, we consider a system with $N=1000$ items, each with a size of $b=10$ and refresh rates $\lambda = 20$. User requests for items follow a Zipf popularity distribution with a parameter of $z=1$, where $p_n$ is proportional to $\frac{1}{n}$. Simulations are conducted under various average cache occupancy constraints, denoted as ${B}$. Fetching cost per item size is represented by $c_f=1$, and aging cost per single age is $c_a = 0.1$. The time averaging parameter $\theta$ is set to $\theta = 0.005$. These parameters will be used throughout the paper unless specified otherwise.
We gauge performance using the percentage cost increase of our proposed model-based learning policy compared to the optimal caching's cost. The percentage cost increase is calculated using:
where $C^{MB}$ is the average long-term cost of the model-based learning policy, and $C^*(\beta,\mathbf{p},\boldsymbol{\lambda})$ denotes the optimal average cost given in Equation \ref{eq:optimalcost_unlimited}, considering unlimited cache capacity and perfect knowledge of the system parameters. Evaluating the cost increase as a percentage allows for effective assessment of the proposed caching policy's performance in terms of cost optimization.
According to Fig. \ref{fig:model-based}, when the cache capacity is unlimited, our proposed caching policy demonstrates a mere 4$\%$ cost increase, approaching optimal performance. This remarkable performance is notable considering that the proposed policy does not possess knowledge of the popularity profile, refresh rates, and demand intensity, unlike the optimal policy.
Furthermore, as the cache size becomes limited, the performance gap between the proposed policy and the optimal strategy slightly increases. However, even in these constrained scenarios, the cost increase remains relatively low, below 10$\%$. As cache size becomes limited, the performance gap slightly widens; however, even in constrained scenarios, the cost increase stays below 10$\%$. This underscores the proposed policy's ability to not only learn popularity and refresh rates but also effectively utilize limited cache capacity, achieving lower average costs.
Our analysis, relying on Poisson process arrivals, led to the development of a model-based caching policy based on Theorem \ref{thm:optimalpolicy}. However, practical scenarios may deviate from the assumption of exponentially distributed interarrival times. To address this, we propose a model-free reinforcement learning approach. This approach allows the system to learn and utilize an optimal policy, regardless of the request arrival distribution. We seek to compare the performance of our model-based policy with the model-free approach in scenarios with diverse request arrival distributions, providing insights into their adaptability and effectiveness.
\section{Comparison to Model-Free Learning} 
In this section, we extend our analysis beyond the Poisson Process assumption, addressing dynamic content caching in a more general context. We consider scenarios where arrival requests don't follow a known distribution, and both update rate and popularity profiles are unknown. To tackle these challenges, we propose a learning approach for caching dynamic content based on Reinforcement Learning, aiming to enhance the efficiency of content delivery in such dynamic environments.
More specifically, we take the Q-Learning approach where the evolution of $Q$'s for each data item $n$ can be expressed as:
In our analysis, we utilize the notations $S_t$, $S_{t+1}$, and $u_t$ to represent the current state, next state, and the action taken at time $t$, respectively. Due to the unavailability of the probability distribution $P(S_{t+1} | S_y, u_t)$, the learning approach we employ is considered model-free. At each time step, there are two potential actions: cache update/fetch, denoted as $u_t = 1$, and no cache update, represented by $u_t = 0$. Using the estimated value for $Q$'s, the optimal action at each state $S_t$ is given by:
Given that the state $S_t$ evolves continuously over time $[0, \infty)$, we discretize time into steps of size $0.1$ seconds before applying the Q-Learning algorithm. 
For a more insightful comparison between the proposed model-based learning (Algorithm 1) and the model-free learning approach, we consider interarrival times of each data item $n$ following a Gamma distribution with parameters $(\omega, \frac{1}{\omega\beta p_n })$. This distribution ensures a constant average interarrival time of $\frac{1}{\beta p_n}$, regardless of $\omega$. The parameter $\omega > 0$ determines the variance, given by $\frac{1}{\omega (\beta p_n)^2}$. When $\omega = 1$, the distribution is equivalent to the exponential distribution. This choice facilitates a meaningful performance comparison between the proposed algorithms.
As a performance metric, we calculate the percentage cost increase of the model-free RL policy compared to the model-based caching policy (Algorithm 1) using the formula:
This metric facilitates an effective comparison of their cost optimization capabilities. Positive values favor Algorithm 1, while negative values favor the RL algorithm. We consider a system with $N=1000$ items, each of size $b=1$, requested uniformly with $p_n=0.001, \forall n$. Refresh rates are $\lambda = 20$. Interarrival times follow a Gamma distribution with parameters $(\omega, \frac{1}{\omega\beta p_n})$, where $\beta = 5$. Varying $\omega$ alters the interarrival time distribution, allowing us to analyze the impact on the performance of the caching algorithms and gain insights into their behavior under different scenarios.
According to Fig. \ref{fig:comparison}, for $\omega=1$, representing exponential interarrival times, Algorithm 1 slightly outperforms RL caching. This result was expected since Algorithm 1 is specifically designed for this type of environment.
Moreover, model-based learning, with faster convergence and less training time, proves competitive to RL caching in scenarios with modest variance. This emphasizes the cost-effectiveness and adaptability of model-based learning, requiring no retraining for environmental changes compared to the resource-intensive retraining needed for RL caching. On the other hand, with significantly reduced $\omega$ (e.g., $\omega = 0.001$), corresponding to large variances, RL caching outperforms model-based caching by almost 50$\%$. However, this improvement comes at the expense of extensive training time.  
In Fig. \ref{fig:omega}, we compare the percentage cost increase of model-free reinforcement learning (given by Equation \ref{eq:percentageRL}) with the model-based policy (given by Equation \ref{eq:percentageMB}) against the optimal solution under the Poisson process assumption. The plot shows these increases as functions of the environment parameter $\omega$ over a $10^6$ seconds duration. Surprisingly, model-based learning, designed for Poisson arrivals, performs nearly as well as model-free RL in more general environments, maintaining high gains as the variance of interarrival times decreases. However, when the variance increases, model-free RL outperforms model-based learning. It's crucial to note that the higher gains of model-free RL come with longer training times and sensitivity to environmental changes, requiring retraining and significant computational resources.
\section{Conclusion}
In conclusion, our study addresses dynamic content caching in scenarios with limited knowledge of item popularity, demand intensity, and refresh rates. For Poisson process arrivals, we unveil a threshold-based optimal policy with complete environmental knowledge and propose a model-based learning algorithm, achieving near-optimal cost without resource-intensive training. We also introduce a Reinforcement Learning (RL) algorithm for more general environments, which outperforms model-based learning in cases with large variance but demands higher computational resources. The choice between model-based learning and model-free RL depends on the environment characteristics. Model-based learning is efficient for moderate variances, while model-free RL achieves better performance in scenarios with substantially large variances, which comes at the cost of longer training times and higher computational demands.
